Self-Guided Masked Autoencoders for Domain-Agnostic Self-Supervised Learning

Self-supervised learning excels in learning representations from large amounts of unlabeled data, demonstrating success across multiple data modalities. Yet, extending self-supervised learning to new modalities is non-trivial because the specifics of existing methods are tailored to each domain, such as domain-specific augmentations which reflect the invariances in the target task. While masked modeling is promising as a domain-agnostic framework for self-supervised learning because it does not rely on input augmentations, its mask sampling procedure remains domain-specific. We present Self-guided Masked Autoencoders (SMA), a fully domain-agnostic masked modeling method. SMA trains an attention based model using a masked modeling objective, by learning masks to sample without any domain-specific assumptions. We evaluate SMA on three self-supervised learning benchmarks in protein biology, chemical property prediction, and particle physics. We find SMA is capable of learning representations without domain-specific knowledge and achieves state-of-the-art performance on these three benchmarks.

==> mask_visualization/pointcloud.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.23\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/guitar_random_masking_visualization.png}
    \caption{\textcolor{red}{Visualization of random masking where masked points are  orange.}}
    \label{fig:image1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/guitar_random_masking_removed_visualization.png}
    \caption{\textcolor{red}{Visualization of random masking with masked points removed.}}
    \label{fig:image2}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/guitar_sma_masking_visualization.png}
    \caption{\textcolor{red}{Visualization of \ours masking where masked points are orange.}}
    \label{fig:image3}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/guitar_sma_masking_removed_visualization.png}
    \caption{\textcolor{red}{Visualization of \ours masking with masked points removed.}}
    \label{fig:image4}
  \end{subfigure}
  \caption{\textcolor{red}{Masking comparison between random masking and \ours on Modelnet40~\cite{modelnet40} pointcloud. We find that \ours obsfucates whole parts of the object such as the top and bottom of the guitar to create a well-defined self-supervision task based on recovering missing components. In comparison random masking just uniformly obsfucates random points which makes for an ill-defined reconstruction task since there is little to distinguish between masked points and points missed during sampling. Best viewed digitally while zooming in.}}
    \label{fig:pointcloud_visualization}
\end{figure}

==> mask_visualization/protein.tex <==

\begin{table*}[t!]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{ll}
            \toprule
            Unmasked Reference & PNPQIDFENSPFYVNSKLSEWKANSNPRRAGVSSFGIGGTNAHLILEEAPTPTVSSPARAQQLLILSAKTNSGLDTATTNLVNYLEQYSEANIADVAYTLQVGRRGFNYRRTIV \\ 
            Random Masking & PNP\maskword{|}I\maskword{|}FEN\maskword{|}PFYVNSKL\maskword{|}EWKA\maskword{|}S\maskword{|}PRRAGVSSFGIG\maskword{|}TNAHL\maskword{|}LEEAPTPTVSSPARAQQLL\maskword{|}LS\maskword{|}KTN\maskword{|}GLDTATTNLVNYLEQ\maskword{|}S\maskword{|}ANI\maskword{|}DVAYTLQVG\maskword{|}RGFN\maskword{|}R\maskword{|}TIV \\
            Learned Mask View 1 & {\maskword{l}\maskword{l}\maskword{l}\maskword{l}}I{\maskword{l}}F{\maskword{l}\maskword{l}\maskword{l}}PFYV{\maskword{l}}SKLSEWKANS{\maskword{l}}PRR{\maskword{l}}GVSSFG{\maskword{l}}GGTNAHLILEEAPTPTVSSPARAQQLLILSAKTNSGLDTATTNLVNYLEQYSEAN{\maskword{l}}A{\maskword{l}\maskword{l}\maskword{l}}YT{\maskword{l}}QVGRRGFNYRRTIV\\
            Learned Mask View 2 & P{\maskword{l}}PQ{\maskword{l}}DFE{\maskword{l}}SP{\maskword{l}\maskword{l}\maskword{l}}NSK{\maskword{l}\maskword{l}\maskword{l}\maskword{l}\maskword{l}}ANS{\maskword{l}}PRR{\maskword{l}}GVSSF{\maskword{l}}IGGTNAHLILEEAP{\maskword{l}}PTVSSPARAQQLLILSAKTNSGLDTATTNLVNYLEQYSEANIADVAYTLQVGRRGFNYR{\maskword{l}}TIV{\maskword{l}}\\
            
           \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Visualization of learned masks on Pfam~\cite{mistry2021pfam} protein modeling dataset.} Masks learned on Pfam are slightly less clustered with respect to position compared to natural language which may suggest that locality represents correlations less.}
    \vspace{-10pt}
    \label{tab:pfam masking visualization}
\end{table*}

==> sec/7_reproducibility_statement.tex <==
\section{Reproducibility Statement}
To ensure our experiments are reproducible, we describe important implementation details in Section~\ref{sec:implementation_details} and list hyperparameters and model configurations in~\cref{tab:bio_hyperparameters,tab:chem_hyperparameters,tab:physics_hyperparameters,tab:image_hyperparameters,tab:language_hyperparameters}.

%Also, we attach an anonymized copy of our source code used to produce experiments in the supplementary materials along with a short sample of pseudo-code that concisely defines our masking method.

==> tables/imagenet100_with_comparison.tex <==
\begin{table*}[tbp]
\centering
\renewcommand\arraystretch{1.0}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ll c cc}
\toprule
Architecture & Pretraining Method & Domain Agnostic & {w/o augmentation} & {w/ augmentation} \\
\midrule
Perceiver~\cite{ioperceiver} & Patch & \xmark & \textbf{79.6} & 84.3 \\
\midrule
ResNet~\cite{he2016deep} & None & \multirow{2}{*}{\cmark} & 72.5 & 78.1 \\
% ResNet~\cite{he2016deep} & Random Quantization~\cite{wu2023randomized} + MoCo-v3~\cite{chen2021mocov3} & & 76.9 & 81.6 \\
ResNet~\cite{he2016deep} & Random Quantization + MoCo-v3 & & 76.9 & 81.6 \\
\midrule
Perceiver~\cite{ioperceiver} & None & \multirow{3}{*}{\cmark} & 52.5 & 62.7 \\
Perceiver~\cite{ioperceiver} & Random & & 77.6 & 85.6 \\
Perceiver~\cite{ioperceiver} & SMA (ours) & & \textbf{78.5} & \textbf{86.1} \\
\bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{
\textbf{Top-1 accuracy transfer learning comparison on ImageNet-100} evaluation set. We consider a setting of both using augmentation and not using augmentation during downstream finetuning. All models are first pretrained for 200 epochs over the training set using different masking methods. We find that our method outperforms random masking both with and without augmentation during downstream classification.
}
\label{tab:imagenet100}
\vspace{-2em}
\end{table*}
